"My Privacy for their Security": Employees' Privacy Perspectives and Expectations when using Enterprise Security Software

Employees are often required to use Enterprise Security Software ("ESS") on corporate and personal devices. ESS products collect users' activity data including users' location, applications used, and websites visited - operating from employees' device to the cloud. To the best of our knowledge, the privacy implications of this data collection have yet to be explored. We conduct an online survey (n=258) and a semi-structured interview (n=22) with ESS users to understand their privacy perceptions, the challenges they face when using ESS, and the ways they try to overcome those challenges. We found that while many participants reported receiving no information about what data their ESS collected, those who received some information often underestimated what was collected. Employees reported lack of communication about various data collection aspects including: the entities with access to the data and the scope of the data collected. We use the interviews to uncover several sources of misconceptions among the participants. Our findings show that while employees understand the need for data collection for security, the lack of communication and ambiguous data collection practices result in the erosion of employees' trust on the ESS and employers. We obtain suggestions from participants on how to mitigate these misconceptions and collect feedback on our design mockups of a privacy notice and privacy indicators for ESS. Our work will benefit researchers, employers, and ESS developers to protect users' privacy in the growing ESS market.

==> 04-Online_Survey.tex <==
\section{Online Survey}
\label{sec:survey}
The primary objective of the survey is to understand how users perceive the data collection practices and corresponding privacy implications while using ESS. 
 \new{We presented the participants with a list of 32 ESS solutions, which were curated from a keyword web search of terms ``endpoint detection'' and ``enterprise security tools'' (see the list in Appendix~\ref{sfl:vendors}). This list was used to assist participants, who also could provide their own if their ESS was not listed. } %, \mm{How this list was made?} \pt{We used a website (perhaps a couple) that listed some popular ESS solutions, would this be important to document because it is more about facilitating the selection for users and I feel with the ``Other'' option, participants had the option to add their own software.} 
 We asked respondents to choose a maximum of three tools that they had experience with, Though respondents may have used more ESS tools. the limit of three allowed us to collect quality feedback without overwhelming the subjects.  %For the surveys, we identified and listed 32\textbf{?} ESS software 


\begin{table}[t]
\caption{Online Survey Respondents' Demographics}
\label{tab:demographicsOnline}
\centering
\small\addtolength{\tabcolsep}{-3.5pt} \renewcommand{\arraystretch}{1.05}
\begin{tabular}{ccccccccc} \hline
\multicolumn{9}{c}{{\bf n = 428}} \\ \hline \hline
\multicolumn{9}{c}{{\bf Gender} } \\
\multicolumn{3}{c}{\emph{Man}}  & \multicolumn{3}{c}{\emph{Woman}}  & \multicolumn{3}{c}{\emph{Other}} \\
\multicolumn{3}{c}{268}    & \multicolumn{3}{c}{160}    &  \multicolumn{3}{c}{-}  \\ \hline  
\multicolumn{9}{c}{{\bf Country} } \\
\multicolumn{3}{c}{\emph{Canada}}  & \multicolumn{3}{c}{\emph{US}}  & \multicolumn{3}{c}{\emph{Other}} \\
\multicolumn{3}{c}{385}    & \multicolumn{3}{c}{38}    &  \multicolumn{3}{c}{5}  \\ \hline
\multicolumn{9}{c}{{\bf Self Reported Proficiency in IT}} \\
\multicolumn{3}{c}{\emph{Basic}} & \multicolumn{3}{c}{\emph{Intermediate}} & \multicolumn{3}{c}{\emph{Advanced}} \\
\multicolumn{3}{c}{65} & \multicolumn{3}{c}{283} & \multicolumn{3}{c}{80}   \\  \hline 
\multicolumn{9}{c}{{\bf Education or Work in IT}} \\
\multicolumn{3}{c}{\emph{No}} & \multicolumn{3}{c}{\emph{Yes}} & \multicolumn{3}{c}{\emph{Undisclosed}} \\
\multicolumn{3}{c}{59} & \multicolumn{3}{c}{366} & \multicolumn{3}{c}{3}   \\  \hline 
\multicolumn{9}{c}{{\bf Highest Education}} \\
\multicolumn{3}{c}{\emph{Undergraduate}} & \multicolumn{2}{c}{\emph{Master's}} & \multicolumn{3}{c}{\emph{Doctoral}} & \multicolumn{1}{c}{\emph{Other}} \\
\multicolumn{3}{c}{183} & \multicolumn{2}{c}{171} & \multicolumn{3}{c}{62} & \multicolumn{1}{c}{12} \\ \hline 
\multicolumn{9}{c}{{\bf Age (in years)}} \\
\emph{18--25}               & \emph{26--30}               & \emph{31--35}               & \emph{36--40}               & \emph{41--45}               & \emph{46--50}               & \emph{50+} & \multicolumn{2}{c}{\emph{Undisclosed}}  \\
59                 & 84                 & 190                 & 52                 & 23                 & 12                  & 6   & \multicolumn{2}{c}{2}\\ \hline
\end{tabular}
\end{table}



 \begin{figure}[t]
    \centering
    \includegraphics[trim={10mm 15mm 15mm 15mm},clip, width=8cm] {figs/reported_use_of_ess_by_respondentes.pdf}
    \caption{Number of times an ESS was reportedly used by survey respondents. ``Other'' includes ESS with ten or fewer selections and unlisted ESS.}
    \label{fig:tool_usage}
\end{figure}



\subsection{Recruitment and Procedure}
\new{Unlike bossware, ESS solutions are primarily used by professionals. Getting participants with a professional background and familiarity  with ESS through public sources (e.g., Facebook Marketplace or Craigslist) is challenging. We resorted to LinkedIn and Facebook through primary and secondary connections and through word-of-mouth. We only directly shared the survey link with professionals.
%We recruited respondents for the online survey by placing advertisements on LinkedIn, Facebook, and through word-of-mouth. %\ch{used facebook but not marketplace, and did not use kijiji} % (see advertisement text in Appendix~\ref{app:recruitment_ad}). 
Our recruitment approach has obvious limitations of convenience sampling, which we discuss further in \S~\ref{subsec:survey_results}}. 

The survey participant criteria necessitated that the respondents currently use a security software provided by their workplace.  Participants responded to the survey on Qualtrics (provided in Appendix~\ref{app:online_survey}). The survey collected data from respondents for the following data categories: (1) Demographics and background; (2) ESS tools used; (3) understanding \st{and comfort} of the data collection by ESS; and (4) perspective on the sufficiency of privacy controls provided by ESS. 
Respondents were asked if they wish to be contacted for a follow-up interview at the end of the survey. Participants were compensated \$5 for the completion of the survey.
%\ch{Category 1 was used to develop an understanding of the background characteristics of the audience reached and ensure that we had a broad array of data to reduce demographic bias. Categories 2, 3 and 4 were composed of strategic questions to answer our previously stated research questions. }

\subsection{Results}
\label{subsec:survey_results}
For test statistics, we use Pearson's Chi-Squared to compare categorical data, a Kruskal-Wallis one-way analysis of variance to compare Likert scale responses between respondents (e.g., their technology proficiency levels), and Wilcoxon Signed-Ranks test to compare Likert scale responses between questions. For multiple comparisons,  we use Bonferroni correction. %\hk{update for tests actually used}


\subsubsection{Demographics and Background}
Respondents were asked about their age, gender, country of residence, level of technology proficiency, \new{industry type and size}, and their education or work background in technology.
The survey was completed by 428 respondents (nine incomplete responses were filtered). Table~\ref{tab:demographicsOnline}  summarizes the demographics of respondents.
The results show a reasonable diversity among respondents in terms of gender. Since the study took place in Canada, the majority of respondents are Canadian. 44\% (190/428) of the respondents are between the ages of 31--35 years, which  captures mid-career professionals. We \new{also have representation from the other age groups: 14\% between 18--25 years, 20\% between 26--30 years, and 12\% between 36--40 years of age}. % The majority age group captures mid-career professionals.
A significant portion of the respondents (65\% (278/428)) self-reported an intermediate proficiency in technology as compared to those who self-reported as basic or advanced proficiency. Similarly, 85\% (364/428) of respondents had education or worked in technology and 54\% (231/428) of respondents had a Master's or a Doctoral degree. 
\new{Respondents reported experience in diverse industries: 43\% (183/428) of participants in technology, 24\% (104/428) in financial, 16\% (68/428) in education, and 13\% (54/428) in science/research industry.}

\new{We note representation from different demographics, different industries, and different organization sizes (reported in \S~\ref{subsec:ess_use}). However, due to our recruitment approach, we observe a large proportion of highly educated and IT focused respondents. This higher representation may also be expected due to the nature of ESS, which are  primarily designed to protect technology resources of the organization.
%This higher representation is likely due to the study being advertised to people who are aware of their ESS use. 
Having more educated participants may help us identify privacy issues that may not be noticeable by less educated or less IT-focused users. On the other hand, the latter group may have misconceptions around privacy in ESS. 
Our work needs to be complemented with future studies that explore ESS perceptions for other population groups.}
%\ch{Ultimately the survey demographics provided us with  suitable \mm{physical = ?} and professional diversity. }

\begin{figure}[t]
    \centering
    \includegraphics[trim={30mm 45mm 10mm 10mm},clip, width=7cm] {figs/Organization_size.pdf}
    \caption{Number of times ESS was reportedly used in organizations of different sizes by survey respondents.}
    \label{fig:organization_size}
\end{figure}

\begin{table}[t]
\caption{\new{Survey responses showing distribution of three information sources on how they communicated regarding what ESS does, features it provides, and data sources it uses for 851 reported user-ESS interactions.}}
\label{tab:channel_source}
\centering
\small\addtolength{\tabcolsep}{-1.0pt} %\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lrrr}
\hline
%\multicolumn{4}{c}{\textbf{n = 842}}       \\ \hline \hline
\multicolumn{4}{c}{\textbf{What it does?}} \\ 
                          & \multicolumn{1}{c}{\textit{ESS}} & \multicolumn{1}{c}{\textit{Employer}} & \multicolumn{1}{c}{\textit{Self}} \\
\textit{No communication} & 8\% (71/851)                               & 8\% (70/851)                                     & 10\% (89/851)                                 \\
\textit{Yes, somewhat}    & 45\% (385/851)                              & 50\% (424/851)                                   & 45\% (381/851)                                \\
\textit{Yes, clearly}     & 45\% (385/851)                              & 41\% (346/851)                                   & 41\% (349/851)                               \\
\textit{Undisclosed}      & 1\% (10/851)                                & 1\% (11/851)                                     & 4\% (32/851) \\ \hline
\multicolumn{4}{c}{\textbf{Feature it provides}} \\ 
                          & \multicolumn{1}{c}{\textit{ESS}} & \multicolumn{1}{c}{\textit{Employer}} & \multicolumn{1}{c}{\textit{Self}} \\
\textit{No communication} & 8\% (64/851)                               & 10\% (84/851)                                    & 12\% (101/851)                               \\
\textit{Yes, somewhat}    & 40\% (337/851)                              & 45\% (386/851)                                    & 43\% (366/851)                               \\
\textit{Yes, clearly}     & 52\% (441/851)                              & 44\% (371/851)                                   & 43\% (370/851)                               \\
\textit{Undisclosed}      & 1\% (9/851)                                & 1\% (10/851)                                     & 2\% (14/851) \\ \hline
\multicolumn{4}{c}{\textbf{Data sources it uses}} \\ 
                          & \multicolumn{1}{c}{\textit{ESS}} & \multicolumn{1}{c}{\textit{Employer}} & \multicolumn{1}{c}{\textit{Self}} \\
\textit{No communication} & 14\% (121/851)                               & 12\% (102/851)                                    & 11\% (92/851)                                \\
\textit{Yes, somewhat}    & 49\% (415/851)                              & 49\% (416/851)                                   & 53\% (447/851)                               \\
\textit{Yes, clearly}     & 36\% (305/851)                              & 38\% (320/851)                                   & 35\% (300/851)                               \\
\textit{Undisclosed}      & 1\% (10/851)                                & 2\% (13/851)                                     & 1\% (12/851) \\ \hline
\end{tabular}
\end{table}
\subsubsection{Reported ESS Use}
\label{subsec:ess_use}
The 428 participants reported 851 unique user to ESS interactions (termed as \emph{user-ESS interaction}).  The distribution of usage across different ESS is reported in Figure~\ref{fig:tool_usage}. All 32 ESS listed were selected by one or more participants. To improve presentation, every ESS with ten or fewer reported usages has been categorized as ``Other''  in Figure~\ref{fig:tool_usage}.  
Cisco AnyConnect Secure Mobility Client, Barracuda CloudGen Access, Cato SASE, and Cisco SASE were the top reported ESS used. Though ESS types fluctuate in use, we note a prominent use of SASE and EDR across participants.
%Participants reported these \emph{user-ESS interactions} occurred 615 times on corporate devices and 479 times on personal devices. 

 %(833/851 provided a response)
%\mm{Got confused between 842 vs 851 vs 833}
\new{For each user-ESS interaction, we inquired about the size of the organization where the ESS was used.. Figure~\ref{fig:organization_size} shows that 11\% (94/851) of the reported user-ESS interactions were from organizations of size 1--10 employees, 37\% (317/851) from 11--50 employees, 31\% (268/851) from 51-100 employees, 11\% (95/851) from 101--500 employees, 2\% (17/851) from 501--1000 employees, 5\% (42/851) from 1000+ employees, and 2\% (18/851) chose not to respond.}

\new{In terms of the target device that ESS was installed on, 41\% (352/851) were reported on corporate devices, 26\% (223/851) were reported on personal devices, and 30\% (255/851) were reported for both corporate and personal devices. 2\% (21/851) interactions did not have this data reported.} \new{68\% (293/428) respondents reported using ESS on at least one personal device.} The usage distribution indicates that a significant proportion of ESS is used on  personal devices, which inevitably resides closely with the personal data of users.

\begin{figure}[t]
   \centering
   \includegraphics[trim={0mm 35mm 5mm 5mm},clip, width=9cm] {figs/only_self_vs_others.pdf}
   \caption{Percentage of ESS-user interactions where respondents reported learning about different data sources using self exploration or through ESS or employer.}%\mm{Change Files scan to File scan - cf. File upload}.}% that received no communication for what the ESS does, feature it provides, and data sources it uses for different organization sizes (interactions have been normalized by the organization size).''}
   \label{fig:self_exploration_only}
\end{figure}



%\begin{figure}[t]
%    \centering
%    \includegraphics[trim={28mm 50mm 5mm 25mm},clip, width=\linewidth] {figs/channel_src.pdf}
%    \caption{Distribution of three information sources (ESS, Employer, Self) on how they communicated (``Yes, clearly'', Yes, somewhat clearly'', ``No (communication)'') regarding what ESS does, features it provides, and data sources it uses.}
%    \label{fig:channel_source}
%\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[trim={0mm 40mm 5mm 5mm},clip, width=9cm] {figs/data_src.pdf}
%    \caption{Distribution of three information sources on whether they communicated about different sources of data collection.}
%    \label{fig:data_source}
%\end{figure}

%\begin{figure*}[t]
 %   \centering
 %   \includegraphics[trim={5mm 25mm 5mm 5mm},clip, width=12cm] {figs/privacy_concerns.pdf}
 %   \caption{Reported comfort of respondents to different activities by ESS.}
 %   \label{fig:privacy_concerns}
%\end{figure*}

\begin{figure*}[t]
   \centering
   \includegraphics[trim={0mm 25mm 5mm 5mm},clip, width=14cm] {figs/percent_no_response.pdf}
   \caption{Percentage of ESS-user interactions that received no communication for what the ESS does, feature it provides, and data sources it uses for different organization sizes (interactions have been normalized by the organization size).''}
   \label{fig:no_response_org_size}
\end{figure*}


\subsubsection{Users' Understanding of Collected Data}
\label{sec:user_understanding_collection}

%\hk{List what sources convey this information to user (Figure \ref{fig:data_source}. List what data types users think is most likely collected (plot current being generated by Jonah).  Later in the discussion section, we want to discuss whether their understanding is correct}
We look at users' understanding of ESS data collection from two perspectives: where do they receive this information from (i.e., information sources) and what is conveyed through these sources. 
First, we consider the informational sources that contribute to the knowledge of users about ESS.  Three information sources of interest for this work include: ESS (e.g., through a privacy notice), employers (e.g., through training), and users' self-exploration (e.g., from online sources or colleagues). In terms of the information conveyed, key aspects include the purpose of software (i.e., what it does---e.g., ``lets me access corporate resources''), features it provides, and data sources that it uses. \newer{We note that respondents' understanding of these aspects may be flawed, and we discuss this limitation further in \S~\ref{sec:limitation}.}

%Figure~\ref{fig:channel_source}
Table~\ref{tab:channel_source} shows whether the three possible information sources (ESS, Employer, and Self), informed users about what the ESS tool does, features it provides, and data sources it uses for 842 reported user-ESS interactions. %\new{We note that although participants reported 872 \emph{user-ESS interaction} only 842 of these \emph{user-ESS interaction} completed these questions.}
% very interesting that the proportions of answers were consistent in all groups with all data sources. i would put intro statement - Overall there is strong correlation of the response for each information source. - what is does seems awkward- could we switch to " understood function" or something clearer
In terms of ``what it does'', for at least 8\% (70/842) of the user-ESS interactions, respondents were  not informed by one of the three sources. 
For 1\% (7/842) user-ESS interactions, five unique respondents received no information about what the ESS does from any source. % (with subtle differences between sources\mm{Explain these differences if important; otherwise delete}). 
For remaining user-ESS interactions, respondents reported learning ``what it does'' (clearly or somewhat clearly) from one or more the three information sources. %\mm{All three? or any of them}. 
We note a similar pattern for the ``provided features''--- at least 8\% (64/842) had no knowledge from one of the information sources. For 1\% (10/842) user-ESS interactions, six unique respondents received no information about the features that the ESS provides from any source.  The remaining user-ESS interactions were informed by one or more of the three sources. %\mm{The discussion on what it does - is somewhat confusing. Please rephrase.} %More participants reported learning about features ``very clearly'' from ESS than the employer or self (441 vs.\ 370). 
For ``data sources it uses'', for at least 11\% (92/842) user-ESS interaction, respondents had no knowledge from one of the three sources.
For 2\% (19/842) user-ESS interactions, twelve unique respondents received no information about the data sources that the ESS provides from any source.
An average of 37\% (314/842) were clearly informed by one or more of the three sources. 

% on the data sources used by ESS.

We note that on average, across the three questions, 50\% (426/842) respondents choose (``Yes, somewhat''), which indicates less certainty about the information that they received.
A Chi-squared test found no significant effect for the three questions about ESS (what ESS does, features it provides, and data sources it uses) and whether they received the information about the question  ($\chi^2(2) = 4.38, p~=~0.11$).

\newer{In Figure~\ref{fig:self_exploration_only}, we report percentage of ESS-user interactions where respondents reported learning about different data sources (e.g., application or location tracking) \mm{The rest is confusing in this sentence - can be rephrased like: using self exploration vs.\ ESS/employer} self exploration (and not through ESS or employer) and through ESS or employer (and not self exploration).
A Bonferroni-corrected Chi-squared test found significant effect for the five data sources and whether they received the information about by self exploration or employer/ESS  ($\chi^2(4) = 52.4, p~<~0.01$).
Post-hoc analysis shows significant differences between ``File upload''/``File Scan'' and others. Respondents were less likely to learn about ``File upload''/``File Scan'' through self exploration.}

\newer{We also report the distribution of user-ESS interactions where the respondents received no information for different organization sizes; see Figure~\ref{fig:no_response_org_size}. The results are reported for the type of information conveyed (i.e., what ESS does, features it provides, and data sources that it uses) and are normalized for the organization size. 
% chi-squared tests for the six organization sizes
Chi-squared tests found significant effect for the organization sizes and whether respondents received no communication ($p~<~0.01$ (Bonferroni-corrected) for all three questions (what ESS does, features it provides, and data sources it uses).
Figure~\ref{fig:no_response_org_size} shows that for organizations with between 11--500 employees, fewer respondents reported receiving no information when compared with organizations with fewer than 10 employees, or over 500 employees (for all three questions). 
While certain factors may explain this difference---e.g., organization type (technology vs.\ manufacturing), less maturity of organizations with fewer than 10 employees, or IT staff preparing the device for organizations with over 500 employees---we did not collect data to find a plausible explanation. This is a possible avenue for a future work.}

%\hk{This figure needs to be explained. @Jonah It would be helpful to have raw numbers here so we can state percentages}


 %\ch{For each listed ESS the survey inquired about the data access requirements on the associated device. The common required data includes file scans, file upload, website traffic, applications, and location. We also wanted understand where the knowledge of these requirements came from so inquired about the information source. This source could have been from self exploration, the employer that required the ESS, and the ESS company itself. The distribution of information source for each data requirement can be seen in Figure \ref{fig:data_source}} 

%For each interaction with ESS, we also asked respondents if one of the three informational sources communicated about the data collection for the following activities by ESS: file scanning, file upload, checking the content of websites, checking the application in use, and tracking the user's location. The results from participants are aggregated in Figure~\ref{fig:data_source}. It shows that the respondents seldom learned about different sources of data by themselves. Between ESS and employers, the employers were more likely to provide information about different sources of data to their employees ($\chi^2(4) = 28.95, p<0.05$). File upload is a notable exception to this trend as the ESS surpasses the employer as the primary information source. %For location tracking the ESS tool itself and the self-exploration both provided equal value to the participants.

\begin{figure}[t]
   \centering
   \includegraphics[trim={0mm 5mm 5mm 5mm},clip, width=9cm] {figs/Provides Privacy.pdf}
   \caption{Survey response to: ``Do you feel that the enterprise security tools, such as the tools you chose previously, provide you with sufficient controls to manage your privacy preferences?''}
   \label{fig:provides_privacy}
\end{figure}

\subsubsection{Privacy  Control's Efficacy}
  \st{To further understand participants perspectives around privacy, first we asked their comfort for each of the five types of data collection activities by ESS on a 5-point Likert scale. These activities include: looking at applications used, websites visited, scanning of personal files, location tracking, and uploading personal files of a user.
Figure} 
%\ref{fig:privacy_concerns} 
\st{shows the responses for each data collection activity. 
For respondents' comfort across five data collection activities, on average 5\% (21/428) reported being not comfortable, 28\% (120/428) slightly comfortable, 34\% (146/428) comfortable, 6\% (26/428) mostly comfortable, and 26\% (111/428) very comfortable, respectively. }% felt ``Slightly Comfortable'' for the aforementioned data sources. \hk{@Jonah confirm numbers}
%on average 5.2\% were not comfortable, 28.4\% were slightly comfortable, 34.4\% comfortable, 7.4\% mostly comfortable, 24.6\% very comfortable felt ``Slightly Comfortable'' for the aforementioned data sources.
\st{The majority of the responses are in the range from ``Comfortable'' to ``Very Comfortable''.} %\pt{This is according to the figure, but I think ``Mostly'' comes before ``Very'' (just a labelling concern\hk{Yes, needs fixing and numbers need to be double checked after fixing})}. 
%Only 3.7\%, 3.9\%, 4.6\%, 5.9\% and 7.8\%
\st{Only a small proportion of participants (8\% (34/428)  or fewer) reported being uncomfortable sharing data related to these five activities.} %\ch{not sure what this sentence is saying} % applications they used, websites they visited, scanning of personal files, location tracking, and upload of their personal files, respectively. 


To understand participants perspectives around privacy controls, we asked respondents if the ESS provides sufficient controls to manage their privacy preferences. %(During the survey design, we debated the use of the term ``controls'' but concluded that it was appropriate for the short survey. We left deeper investigation of control preference for the interview.) 
Their responses on a 5-point Likert scale (``Strongly Disagree'' to ``Strongly Agree'') are shown in Figure
~\ref{fig:provides_privacy}
. It shows that 54\% (231/428) strongly agree or agree, 37\% (158/428) are neutral, and 9\% (39/428) disagree or strongly disagree that ESS provides sufficient controls to manage their privacy preferences. %\mm{We should discuss this perhaps - 9\% here vs.\ what is revealed in the interviews.}
A Kruskal-Wallis test examined the effect of respondent technical proficiency on whether they feel that ESS provides sufficient controls to manage their privacy and found no significant differences ($H(X) = 1.73, p~=~0.42$).

%\ch{Results of this portion showed a promising level of comfort from participants. This group should not negate the population that did not hold the same confidence. This discussion is also subject to some limitations (such as misinterpretation), so will be re-evaluated in depth during the interview portion of this work. }\mm{This para is somewhat ambiguous - too many "this". Please update. This portion = ? This group = ? This discussion = ?} 

%A Chi-squared test found (no?) significant effect for technical proficiency (basic, intermediate and advanced) and whether they feel that ESS provides sufficient controls to manage their privacy ($\chi^2(2) = X.XX, p~=~0.XX$)
%A Wilcoxon Signed-Ranks test indicated that likelihood ratings for an expert attacker were significantly higher than the likelihood ratings for an average attacker ($Z = 8.31, p < 0.001$). 

%54.3\% Agree or strongly agree, 36.9\% neutral, 8.8\% disagree or strongly disagree. %Figure \ref{fig:provides_privacy} emplifies that majority of the respondents agree or are neutral about our question. Conversely, the entire set of participants who disagree account for the smallest share of the distribution. When the latter is combined with the neutral respondents, they account for nearly half of the participants.






==> aux_material.tex <==
%Copying material post methodology and results here. Will copy as needed\ch{I feel like this blurb is not important for final paper.. maybe can talk about the value of the mixed method data in discussion} This mixed-model approach will help to provide both quantitative and qualitative insight on the perspective of professionals, which will be essential for providing accurate reports on our initial propositions. 


As an incentive for participation, we will offer a \$5 compensation for completing the recruitment survey and a guaranteed \$20 for participation in the semi structured interview, as well as raffle entry for a 64GB Apple iPad (valued at CAD \$425+tax). \hk{Say why two-part study. Also have a quick look at the Used devices paper by Jason and me as an example on how to structure this section}

In unison, these results can help guide developers of ESS in improving the usability of their systems. A particular focus will be placed on doing so in a manner that is conducive to delivering their goals while protecting employee's privacy on their own devices brought to the workplace.

Both components require approval from the University of Guelph's Research Ethics Board (REB), so documents were developed early in the research process for submission. 

\subsection{Recruitment Survey}
\ch{flow edited}\hk{I see that you are providing good rationale. It would read nicely when the flow is fixed} 

We began our study with an approximately 10-minute recruitment survey, seeking professionals as participants by way of an invitation through their communication channels and through advertisement on  various social media websites. From this survey we will gain intel regarding the employees' knowledge of ESS such as Okta and Netskope, see \cite{okta_okta_2021, netskope_homepage_2021}. To certify legitimacy, we will provide the participants with a concise introduction explaining our identifications and the purpose of research \cite{ball_conducting_2019}. 

\ch{include info on how we deploy survey}

When developing the survey we compiled a list of questions that directly related to the goal of our study. The leading questions include details such as industry knowledge and experience, which provide us with insight to the reasoning for the participants perspective. The later questions are compiled of organization and personal knowledge of specific software, to gain a deeper understanding of participants information sources and level of knowledge. 

The ESS features described the software websites which were used to create the comprehensive functionality and permissions lists included in the survey have been included in Appendix \ref{sfl}. Additionally, we consulted with media and peers in the industry to ensure current and complete lists. 

To finalize the survey we placed specific ``trigger'' questions to monitor and carry on to discussion for the interview stage. During the entire process, the team referred to the target questions to help guide and prioritize questions to be included in the survey. 

The responses of these participants will be sorted using pre-established selection criteria and then a select group will be invited to the next phase, a semi-structured interview. Only the participants with sufficient experience using ESS and expressed interest in further participating will be invited to the interview. 

\subsection{Semi-Structured Interview}

The goals of the paper were consulted to inform the research questions of this interview phase, with a particular emphasis on garnering insight on a participant's perspective and ideas for improving ESSs. These interviews will have a duration of approximately an hour, which was decided in consideration of providing a more in-depth understanding of the participant's experiences and their time commitments.

The question framework was designed to be flexible to allow for natural conversation, and remain unbiased to seek the participant's true perspective with minimal influence. The discussion was arranged to follow the end-to-end process of using the software, starting with installation, knowledge, current behaviour, and finally perspectives on solutions. The interviewer will have prepared for the interview and researched the ESS listed in the participants survey to specify the questions.
The interview is then directed to elicit the participant's thoughts on the futures of ESS and their preference on addressing their concerns. 

\subsubsection{Interface Prototypes}
\ch{should we have a section regarding this }

A newer addition to the semi-structured interviews was the development of interface prototypes to help people utilize and provide feedback on concrete potential solutions to help bring awareness amongst employees of the powers beholden to ESS. These mockups are inspired by the permission models described in the Background \ref{background:permissions} section in addition to the interfaces presented to users when using apps found in platforms like Facebook.

\subsection{Pilot Studies}
To test the efficacy of the prepared research models pilot studies were conducted with individuals in industry. The study was completed with each pilot study participant with the intention of testing the survey and interview formats in an effort to acquire first-hand feedback from them.

Time stamped copies of the survey and the semi-structured interview documents were retained to track the changes made after each pilot study. By doing this we gained insight to what topic areas were proving to hold importance and where to focus further attention. 
%-------------------------------------------------------------------------------
\section{Results}
%-------------------------------------------------------------------------------


\subsection{Pilot Studies}
The pilot studies served as a successful way to validate and improve our research tools. We learned from each of the pilot studies ways to enhance our survey and our interview questions to better answer our initial research propositions.

\subsection{Recruitment Survey}
From the pilot runs of our recruitment survey, we streamlined the questions to be more easily interpretable by the participants. The survey format was revised \mm{Not sure - but should we add some examples here on how questions were revised?} to make sure the topics of each question were conveyed effectively.  We worked through the questions to make sure that each was worded correctly that the participant would understand the meaning of each question in addition to \mm{the desirable duration = ?}. Eventually, we achieved a wording and flow that maintained the integrity of the questions while allowing for simple interpretation by the user. During this process, we were able to identify redundant questions and shorten the survey to deliver a better experience for the participants. 

With the results of the recruitment survey we will \mm{Mixing past and future tenses..} include a table with the percentages of different demographic information collected. 
We will also show the frequencies of different industries, computer proficiency levels, as well as company sizes. This data is conducive to providing a ratio of knowledge compared to ESS used by the participants. There will also be some information regarding the frequencies of the security tools selected. \ch{QUESTION: would it be interesting to show the ratio of knowledge and the sources for each software? } \pt{Yes!} 

This data will provide an understanding of the general background of participants which may give light to the reasoning of their knowledge level. 

- Pick data from a couple questions that appear in both studies

\subsection{Semi-Structured Interview}
- Some of these ESS gather more data than the employees thought, even those who were responsible for deploying the ESS (P1)

Early pilot testing of the semi-structured interview allowed us to gain a better understanding of present knowledge gaps and reform our questions to better communicate with the participants. Initial conversation with the participants allowed us to alter the questions to accommodate for the knowledge level of the participant. These changes allowed for the conversation within the interview to flow better, which resulted in better feedback from the participants.

\ch{im not 100\% set on this.. please review and let me know if it works :) 


With the quantified responses from the interview questions we will be able to  compartmentalize the questions relating to each of our propositions. Using factor analysis we can determine the variance and covariance of each of the variables which will allow us to further understand causation as well as reduce some of the dimensionality to provide a simpler understanding \cite{noauthor_factor_nodate}.

}

With the qualitative responses we will be able to gain a deeper understanding of the perspectives and knowledge gaps of the participants, among other nuances involved in the deployment of ESS. From this we can collaborate to produce a comprehensive review of the prominent take aways and produce some future steps. One of the fascinating results revealed by a pilot study participants was that organizations may not even themselves be aware of the full extent of the capabilities of the ESS, a perspective we had not previously considered.

The synergy of the quantitative and qualitative responses from participants will better articulate the important discussion points that occurred in the survey in addition to providing a better overall understanding of the implications of ESS relative to our propositions.


%%%DISCUSSION
Previous research examined in detail in section \ref{background}, \emph{Background}, has provided a strong foundation for understanding both perspectives of employee surveillance tools. As ESS has advanced and WFH has become more common there was a need to update these research areas. There have been publications discussing the benefits of the modern ESS supporting implementation by employers. Media articles have discussed the implications of ESS \cite{chant_zuckerbergs_2021, chant_uber_2021,  matyszczyk_microsoft_2021}, but little academic work has been done to evaluate the end user perspective. This work has contributed to this area by gaining first-hand feedback from these users in a professional working environment. 

\subsection{Recruitment Survey}
- Describe changes brought abound from pilot study

One of the most prominent changes to the survey that came from pilot testing was the wording of questions and the flow. We noticed that many participants had little idea of what we were asking and many of the questions were misunderstood. From this we were able to recognize that there was less knowledge than we had initially anticipated, both from their employer and in general. In addition, initially, if a participant had no prior knowledge, the survey come abruptly to and end, instead the new iteration entices them to think about their knowledge of the software in different contexts. Another aspect that was improved was the process for recruiting participants for the next phase and provide findings. Through several iterations, the flow was improved to the point where it makes it more trivial for people to independently or collectively select these two aspects of our study. Finally, the various sections of the survey have been divided to clarify which part of the survey they are completing, essential when looping through responses for each software selected.

\subsection{Semi-Structured Interview}
- Describe changes brought abound from pilot study
- This is definitely unanticipated and has the potential to violate the trust of both the organization and the employee, may have resulted from lack of transparency/communication from the ESS developers \cite{kropp_future_2019, nazari_more_2019}

The pilot studies of the semi-structured interview had similar results as the survey. As we continued through the pilot studies, we refined our technique for collecting notes, starting from adding independent notes written along with the questions. This quickly turned into employing Qualtrics XM to collect answers, akin to the survey but with more opportunities to provide insight. However, we plan to use a spreadsheet for future data collection for its potential for changing and reusing answers more swiftly than the previous approach, we feel this will be more conducive to better discussions with the participant. As for the most surprising result, we did not envision the potential for ESS developers to violate the trust of both the employee and the organization, which may have resulted from lack of transparency/communication from the developers \cite{kropp_future_2019, nazari_more_2019}.

From our first pilot we found that there was some confusion when asking about specifics of the ESS. Moving forward we understood that it was necessary to ask about whether they had previous knowledge before continuing to the more specific questions. In addition, a plethora of additional questions to help further guide the interview have been added.

During the second pilot we implemented these techniques and the initial flow was improved and better discussion was sparked. We found that the participant had little knowledge in the differences of the ESS so when we asked questions specifically pertaining to one software then another, there was some repetition and the flow was lost. Moving forward we will inquire about the knowledge of the differences between each software to ensure that the redundancies are removed. 
